Coexistence of Real-Time Source Reconstruction and Broadband Services Over Wireless Networks

Achieving a flexible and efficient sharing of wireless resources among a wide range of novel applications and services is one of the major goals of the sixth-generation of mobile systems (6G). Accordingly, this work investigates the performance of a real-time system that coexists with a broadband service in a frame-based wireless channel. Specifically, we consider real-time remote tracking of an information source, where a device monitors its evolution and sends updates to a base station (BS), which is responsible for real-time source reconstruction and, potentially, remote actuation. To achieve this, the BS employs a grant-free access mechanism to serve the monitoring device together with a broadband user, which share the available wireless resources through orthogonal or non-orthogonal multiple access schemes. We analyse the performance of the system with time-averaged reconstruction error, time-averaged cost of actuation error, and update-delivery cost as performance metrics. Furthermore, we analyse the performance of the broadband user in terms of throughput and energy efficiency. Our results show that an orthogonal resource sharing between the users is beneficial in most cases where the broadband user requires maximum throughput. However, sharing the resources in a non-orthogonal manner leads to a far greater energy efficiency.

==> bib.tex <==
%%%% MIMO

@ARTICLE{Kan22,
  author={Kang, Justin and Yu, Wei},
  journal={IEEE Transactions on Communications}, 
  title={Scheduling Versus Contention for Massive Random Access in Massive {MIMO} Systems}, 
  year={2022},
  volume={70},
  number={9},
  pages={5811-5824},
  doi={10.1109/TCOMM.2022.3190904}}


%%%% Heterogeneous

%and Gimenez-Guzman, Jose Manuel and Valentini, Lorenzo and Popovski, Petar
@INPROCEEDINGS{Ley23Asilomar,
  author={Leyva-Mayorga \textit{et al}., Israel},
  booktitle={Proc. 57th Asilomar Conf. on Signals, Systems, and Computers}, 
  title={Heterogeneous Radio Access with Multiple Latency Targets}, 
  year={2023},
  volume={},
  number={},
  pages={80-84},
  doi={10.1109/IEEECONF59524.2023.10476965}}

@article{Inter24,
      title={On the Coexistence of {eMBB} and {URLLC} in the Cell-Free Massive {MIMO} Downlink}, 
      author={Giovanni Interdonato and Stefano Buzzi},
      note = {arXiv:2405.07585},
      year={2024},
      eprint={2405.07585},
      archivePrefix={arXiv},
      primaryClass={cs.IT}
}

%%%% Cell-free

@ARTICLE{Zha20,
  author={Zhang, Jiayi and Björnson, Emil and Matthaiou, Michail and Ng, Derrick Wing Kwan and Yang, Hong and Love, David J.},
  journal={IEEE Journal on Selected Areas in Communications}, 
  title={Prospective Multiple Antenna Technologies for Beyond {5G}}, 
  year={2020},
  volume={38},
  number={8},
  pages={1637-1660},
  doi={10.1109/JSAC.2020.3000826}}

@ARTICLE{Got24,
  author={Göttsch, Fabian and Osawa, Noboru and Kanno, Issei and Ohseki, Takeo and Caire, Giuseppe},
  journal={IEEE Transactions on Wireless Communications}, 
  title={Fairness Scheduling in User-Centric Cell-Free Massive {MIMO} Wireless Networks}, 
  year={2024},
  note={early access},
  number={},
  pages={1-1},
  doi={10.1109/TWC.2024.3386802}}

@article{Ngo24,
      title={Ultra-Dense Cell-Free Massive {MIMO} for {6G}: Technical Overview and Open Questions}, 
      author={Hien Quoc Ngo and Giovanni Interdonato and Erik G. Larsson and Giuseppe Caire and Jeffrey G. Andrews},
      year={2024},
      note={arXiv: 2401.03898}}



%%%% NOMA
@article{Vaezi2019,
   author = {Mojtaba Vaezi and Robert Schober and Zhiguo Ding and H. Vincent Poor},
   doi = {10.1109/MWC.2019.1800598},
   issn = {1536-1284},
   issue = {5},
   journal = {IEEE Wireless Communications},
   month = {10},
   pages = {174-180},
   publisher = {IEEE},
   title = {Non-Orthogonal Multiple Access: Common Myths and Critical Questions},
   volume = {26},
   year = {2019},
}


%%%% Feedback and scheduling

@ARTICLE{Kang2020,
  author={Kang, Justin and Yu, Wei},
  journal={IEEE Transactions on Information Theory}, 
  title={Minimum Feedback for Collision-Free Scheduling in Massive Random Access}, 
  year={2021},
  volume={67},
  number={12},
  pages={8094-8108},
  doi={10.1109/TIT.2021.3114584}}



%%%%    Timing metrics: AoI and AOII
@ARTICLE{Maatouk20,
  author={Maatouk, Ali and Kriouile, Saad and Assaad, Mohamad and Ephremides, Anthony},
  journal={IEEE/ACM Transactions on Networking}, 
  title={The Age of Incorrect Information: A New Performance Metric for Status Updates}, 
  year={2020},
  volume={28},
  number={5},
  pages={2215-2228},
  doi={10.1109/TNET.2020.3005549}}

@INPROCEEDINGS{Yates21,
  author={Yates, Roy D.},
  booktitle={Proc. IEEE International Symposium on Information Theory (ISIT)}, 
  title={The Age of Gossip in Networks}, 
  year={2021},
  volume={},
  number={},
  pages={2984-2989},
  keywords={Measurement;Protocols;Observers;Tools;Complexity theory;Energy harvesting;Information theory},
  doi={10.1109/ISIT45174.2021.9517796}}

@article{Salimnejad24_arxiv,
      title={Version Innovation Age and Age of Incorrect Version for Monitoring Markovian Sources}, 
      author={Mehrdad Salimnejad and Marios Kountouris and Anthony Ephremides and Nikolaos Pappas},
      year={2024},
      note={2401.17691},
      archivePrefix={arXiv},
      primaryClass={cs.IT}
}

@ARTICLE{Salimnejad_tcom,
  author={Salimnejad, Mehrdad and Kountouris, Marios and Pappas, Nikolaos},
  journal={IEEE Transactions on Communications}, 
  title={Real-Time Reconstruction of Markov Sources and Remote Actuation Over Wireless Channels}, 
  year={2024},
  volume={72},
  number={5},
  pages={2701-2715},
  doi={10.1109/TCOMM.2024.3356456}}


%%%% ISAC

@ARTICLE{Trev23,
  author={Trevlakis, Stylianos E. and Boulogeorgos, Alexandros-Apostolos A. and Pliatsios, Dimitrios and Querol, Jorge and Ntontin, Konstantinos and Sarigiannidis, Panagiotis and Chatzinotas, Symeon and Di Renzo, Marco},
  journal={IEEE Open Journal of the Communications Society}, 
  title={Localization as a Key Enabler of {6G} Wireless Systems: A Comprehensive Survey and an Outlook}, 
  year={2023},
  volume={4},
  number={},
  pages={2733-2801},
  doi={10.1109/OJCOMS.2023.3324952}}

@INPROCEEDINGS{Zabini22,
  author={Zabini, Flavio and Paolini, Enrico and Xu, Wen and Giorgetti, Andrea},
  booktitle={Proc. IEEE Global Communications Conference (GLOBECOM)}, 
  title={Joint Sensing and Communications in Finite Block-Length Regime}, 
  year={2022},
  volume={},
  number={},
  pages={5595-5600},
  doi={10.1109/GLOBECOM48099.2022.10001119}}


%%%% Matching
@ARTICLE{Gu15,
  author={Gu, Yunan and Saad, Walid and Bennis, Mehdi and Debbah, Merouane and Han, Zhu},
  journal={IEEE Communications Magazine}, 
  title={Matching theory for future wireless networks: fundamentals and applications}, 
  year={2015},
  volume={53},
  number={5},
  pages={52-59},
  keywords={Resource management;Wireless networks;Algorithm design and analysis;Cellular networks;Cognitive radio;Interference},
  doi={10.1109/MCOM.2015.7105641}}

@article{Avis83,
author = {Avis, David},
title = {A survey of heuristics for the weighted matching problem},
journal = {Networks},
volume = {13},
number = {4},
pages = {475-493},
year = {1983}
}

@article{Kuhn55,
author = {Kuhn, H. W.},
title = {The {Hungarian} method for the assignment problem},
journal = {Naval Research Logistics Quarterly},
volume = {2},
number = {1-2},
pages = {83-97},
year = {1955}
}

@INPROCEEDINGS{pappas@dtmc,
  author={Pappas, Nikolaos and Kountouris, Marios},
  booktitle={Proc. IEEE Int. Conf. on Autonomous Systems (ICAS)}, 
  title={Goal-Oriented Communication For Real-Time Tracking In Autonomous Systems}, 
  year={2021},
  volume={},
  number={},
  pages={1-5},
  keywords={Wireless communication;Measurement;Costs;Autonomous systems;Transmitters;Semantics;Markov processes;Goal-oriented communication;semantics of information;cost of actuation error;real-time tracking.},
  doi={10.1109/ICAS49788.2021.9551200}}


%and Leyva-Mayorga, Israel and Stefanovi\'{c}, \v{C}edomir and Kal\o{r}, Anders E. and Popovski, Petar}
@ARTICLE{OJCOMMS@fedrico,
  author={Chiariotti \textit{et al}., Federico},
  journal={IEEE Open Journal of the Communications Society}, 
  title={{RAN} Slicing Performance Tradeoffs: Timing Versus {Throughput} {Requirements}}, 
  year={2022},
  volume={3},
  number={},
  pages={622-640},
  keywords={NOMA;Broadband communication;Throughput;Time division multiple access;Timing;Uplink;Frequency division multiaccess;Age of information (AoI);heterogeneous services;non-orthogonal multiple access (NOMA);reliability;slicing},
  doi={10.1109/OJCOMS.2022.3164733}}

@ARTICLE{pappas@dtmcTWC,
  author={Salimnejad, Mehrdad and Kountouris, Marios and Pappas, Nikolaos},
  journal={IEEE Transactions on Communications}, 
  title={Real-Time Reconstruction of Markov Sources and Remote Actuation Over Wireless Channels}, 
  year={2024},
  volume={72},
  number={5},
  pages={2701-2715},
  keywords={Real-time systems;Receivers;Measurement;Markov processes;Costs;Monitoring;Wireless communication;Goal-oriented semantics-aware communications;real-time tracking;cost of actuation error;timing-aware error metrics},
  doi={10.1109/TCOMM.2024.3356456}}


@inproceedings{WEIMER2012178,
title = {Distributed Event-Triggered Estimation in Networked Systems},
booktitle = {Proc. IFAC Conference on Analysis and Design of Hybrid Systems},
volume = {45},
number = {9},
pages = {178-185},
year = {2012},
issn = {1474-6670},
doi = {https://doi.org/10.3182/20120606-3-NL-3011.00099},
author = {James {Weimer, \textit{et al}.}},
keywords = {Distributed Event-Triggered, State Estimation, Networked Systems},
}


@ARTICLE{Sun@AoI,
  author={Sun, Yin and Polyanskiy, Yury and Uysal, Elif},
  journal={IEEE Transactions on Information Theory}, 
  title={Sampling of the Wiener Process for Remote Estimation Over a Channel With Random Delay}, 
  year={2020},
  volume={66},
  number={2},
  pages={1118-1135},
  keywords={Information age;Estimation error;Silicon;Real-time systems;Channel estimation;Servers;Sampling;remote estimation;age of information;Wiener process;queuing system},
  doi={10.1109/TIT.2019.2937336}}

@ARTICLE{Pappas@SmeanticsMagazine,
  author={Kountouris, Marios and Pappas, Nikolaos},
  journal={IEEE Communications Magazine}, 
  title={Semantics-Empowered Communication for Networked Intelligent Systems}, 
  year={2021},
  volume={59},
  number={6},
  pages={96-102},
  keywords={Wireless communication;Correlation;Semantics;Distributed databases;Real-time systems;Distributed databases},
  doi={10.1109/MCOM.001.2000604}}

%and Chiariotti, Federico and Huang, Kaibin and Kalør, Anders E. and Kountouris, Marios and Pappas, Nikolaos and Soret, Beatriz
@ARTICLE{TimePerspective@Popovski,
  author={Popovski \textit{et al}., Petar },
  journal={Proceedings of the IEEE}, 
  title={A Perspective on Time Toward Wireless {6G}}, 
  year={2022},
  volume={110},
  number={8},
  pages={1116-1146},
  keywords={Complexity theory;Wireless communication;Real-time systems;6G mobile communication;Ultra reliable low latency communication;5G mobile communication;Wireless sensor networks;Next generation networking;Systematics;Receivers;6G mobile communication;cellular technology;low latency communication;real-time systems},
  doi={10.1109/JPROC.2022.3190205}}

@ARTICLE{Anup@6G,
  author={Mishra \textit{et al}., Anup},
  journal={IEEE Communications Letters}, 
  title={{Rate-Splitting Multiple Access for 6G—Part I: Principles, Applications and Future Works}}, 
  year={2022},
  volume={26},
  number={10},
  pages={2232-2236},
  keywords={Downlink;Multiaccess communication;Uplink;6G mobile communication;NOMA;Transceivers;Time-frequency analysis;Next generation multiple access (NGMA);rate-splitting multiple access (RSMA);6G},
  doi={10.1109/LCOMM.2022.3192012}}

@article{Chiariotti2021,
author = {Chiariotti, Federico and Leyva-Mayorga, Israel and Stefanovi\'{c}, {\v{C}}edomir and Kal{\o}r, Anders E. and Popovski, Petar},
doi = {10.3390/e23060686},
journal = {Entropy},
month = may,
number = {6},
pages = {686},
title = {{Spectrum Slicing for Multiple Access Channels with Heterogeneous Services}},
volume = {23},
year = {2021}
}
